Towards Performance Clarity of Edge Video Analytics

Edge video analytics is becoming the solution to many safety and management tasks. Its wide deployment, however, must first address the tension between inference accuracy and resource (compute/network) cost. This has led to the development of video analytics pipelines (VAPs), which reduce resource cost by combining DNN compression/speedup techniques with video processing heuristics. Our measurement study on existing VAPs, however, shows that today's methods for evaluating VAPs are incomplete, often producing premature conclusions or ambiguous results. This is because each VAP's performance varies substantially across videos and time (even under the same scenario) and is sensitive to different subsets of video content characteristics. We argue that accurate VAP evaluation must first characterize the complex interaction between VAPs and video characteristics, which we refer to as VAP performance clarity. We design and implement Yoda, the first VAP benchmark to achieve performance clarity. Using primitive-based profiling and a carefully curated benchmark video set, Yoda builds a performance clarity profile for each VAP to precisely define its accuracy/cost tradeoff and its relationship with video characteristics. We show that Yoda substantially improves VAP evaluations by (1) providing a comprehensive, transparent assessment of VAP performance and its dependencies on video characteristics; (2) explicitly identifying fine-grained VAP behaviors that were previously hidden by large performance variance; and (3) revealing strengths/weaknesses among different VAPs and new design opportunities.

==> edits.tex <==
%!TEX root = benchmarking.tex
%!TEX spellcheck = en_US 


\jc{
\begin{itemize}
\item a concrete example of how an existing VAP 
won't work when there is new demand and how Yoda 
could help improve the VAP design to fit the new 
setting.
=> writing
\item eval results are limited to two settings. 
=> zhengxu's new results
\item reflect diff design goals, like bandwidth 
adaptation => writing, but possibly a new graph?
\item would be nice to discuss impact of net infra
(4g, 5g, etc) => add writing
\item only applicable to 5 pipelines
=> add new pipelines + more writing
\item unfair comparison (related to different 
design goals). other techniques are not discussed, 
like data mngmnt, etc => writing on scope
\item lack real implementation (only emulation) 
=> writing to explain why it's real
\item no network cost (is it true?)
\item clear def of features and primitives => 
writing
\item independence doesn't always hold. => 
better writing + zhujun's new results
\item may not be future proof => better writing
\item doesn't consider inference delay => writing
\item features and primitives are not complete
=> writing. 
\item eval data set only covers a limited number 
of features.. => need to clarify
\end{itemize}
}



\fixme{
Overview of key modifications:
\begin{itemize}
\item	Clarify our problem statement, especially in introduction, to better define “performance clarity” and present the motivation for achieving “performance clarity.”

\item	Explicitly clarity the difference between our work and previous efforts, especially in introduction and related work sections. 

\item	Explicitly define the various terminologies early in the paper (using a table) to provide context and clarity. 
\item	Elaborate the implementation details, including latency regarding fast feature scanning, and ways to find/select representative benchmark videos. 
\item	Add new results about Yoda’s profiling overhead, and explain how we select test videos in evaluating Yoda. 
\end{itemize}
}
